Benchmarking Optimizers for Qumode State Preparation with Variational Quantum Algorithms

Quantum state preparation involves preparing a target state from an initial system, a process integral to applications such as quantum machine learning and solving systems of linear equations. Recently, there has been a growing interest in qumodes due to advancements in the field and their potential applications. However there is a notable gap in the literature specifically addressing this area. This paper aims to bridge this gap by providing performance benchmarks of various optimizers used in state preparation with Variational Quantum Algorithms. We conducted extensive testing across multiple scenarios, including different target states, both ideal and sampling simulations, and varying numbers of basis gate layers. Our evaluations offer insights into the complexity of learning each type of target state and demonstrate that some optimizers perform better than others in this context. Notably, the Powell optimizer was found to be exceptionally robust against sampling errors, making it a preferred choice in scenarios prone to such inaccuracies. Additionally, the Simultaneous Perturbation Stochastic Approximation optimizer was distinguished for its efficiency and ability to handle increased parameter dimensionality effectively.

==> Commented_Content.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figure/error_over_layer.pdf} 
%     \caption{State Preparation Error for Non-Gaussain State over Layers}
%     \label{fig:example}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/Training_error_stochastic_compare.png} 
%     \caption{Training Process for stochastic and non-Stochastic simulation}
%     \label{fig:example}
% \end{figure}
% The specified target state is [0,0,3,4,5,4,3,0,0,0]. The outcome indicates that when utilizing only one layer of the basis gate set, our ansatz tends to converge towards a Gaussian local gate. Two layers are usually enough to learn the Gaussian non local state which is less than the 10 layers required for non Gaussian state. In the initial layer, certain optimizers exhibit sensitivity to barren plateaus. Across 50 trials, the optimization process yields two distinct sets of parameters, characterized by fidelity values around $0.107$ and $0.493$, respectively. For CG and L-BFGS-B optimizer, the distribution of results among these fidelity values is approximately $20\%$ for $0.493$ and $80\%$ for $0.107$. For Nelder-Mead optimizer, the distribution is approximately $30\%$ for $0.493$ and $70\%$ for $0.107$. For COBYLA and Powell optimizer, the distribution is approximately $10\%$ for $0.493$ and $90\%$ for $0.107$. \par 
% For more than one layer,  we employed the Simultaneous Perturbation Stochastic Approximation (SPSA) optimizer to address the challenges posed by the high-dimensional nature of the problem.


% \begin{table}[htbp]
%     \centering
%     \caption{Optimizer Performance for Non Local Gaussian State with Layer = 1}
%     \label{tab:optimizers}
%     \begin{tabular}{lcc}
%     \hline
%     \textbf{Optimizer} & \textbf{Infidelity} & \textbf{Function Evaluations} \\
%     \hline
%     Conjugate Gradient & 0.1840 & 151 \\
%     L-BFGS-B & 0.1807 & 251 \\
%     COBYLA & 0.1456 & 145 \\
%     Nelder-Mead & 0.2231 & 206 \\
%     Powell & 0.1457 &  322 \\
%     \hline
%     \end{tabular}
%     \end{table}
% \begin{table}[htbp]
%     \centering
%     \caption{Optimizer Performance for Non Local Gaussian State with Layer = 2}
%     \label{tab:optimizers}
%     \begin{tabular}{lcc}
%     \hline
%     \textbf{Optimizer} & \textbf{1 - Fidelity} & \textbf{Function Evaluations} \\

%     \hline
%     Conjugate Gradient & xx & xx \\
%     L-BFGS-B & 0.xx & xx \\
%     COBYLA & 0.xx & xx \\
%     Nelder-Mead & 0.xx & xx \\
%     Powell & 0.xx &  xx \\
%     \hline
%     \end{tabular}
%     \end{table}
% \begin{figure*}[htbp]
%   \centering
%     \begin{subfigure}[b]{0.30\textwidth}
%     \includegraphics[width=\textwidth]{figure/Gaussian_non_local/learnt_1layer_G_non_local.png}
%     \caption{Learnt State layer = 1}
%     \label{fig:sub1}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.30\textwidth}
%     \includegraphics[width=\textwidth]{figure/Gaussian_non_local/Learnt_2layer_G_non_local.png}
%     \caption{Learnt State layer = 2}
%     \label{fig:sub1}
%   \end{subfigure}
%   % \hfill
%   \begin{subfigure}[b]{0.30\textwidth}
%     \includegraphics[width=\textwidth]{figure/Gaussian_non_local/target_G_non_local.png}
%     \caption{Target Gaussian Non-Local State}
%     \label{fig:sub2}
%   \end{subfigure}
%   \caption{Wigner Function of Learnt Stat at different Layer for Gaussian Non Local State}
%   \label{fig:main}
% \end{figure*}


% \begin{table}[htbp]
%     \centering
%     \caption{Optimizer Performance for Local Gaussian State}
%     \label{tab:optimizers}
%     \begin{tabular}{lcc}
%     \hline
%     \textbf{Optimizer} & \textbf{Infidelity} & \textbf{Function Evaluations} \\
%     \hline
%     Conjugate Gradient & 0.0262 & 305 \\
%     L-BFGS-B & 0.0248 & 253 \\
%     COBYLA & 0.0246 & 119 \\
%     Nelder-Mead & 0.0252 & 425 \\
%     Powell & 0.0241 &  812 \\
%     \hline
%     \end{tabular}
% \end{table}

% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figure/Gaussian_1layer.png}
%     \caption{Learnt State layer = 1}
%     \label{fig:sub1}
%   \end{subfigure}
%   % \hfill
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figure/target_Gaussian.png}
%     \caption{Target State}
%     \label{fig:sub2}
%   \end{subfigure}
%   \caption{Wigner Function of Learnt Gaussian State}
%   \end{figure}

% In stochastic simulation, we simulate experimental sampling into the measurement outcome, altering the nature of our objective function evaluation from a static reflection. We didn't observe a significant decrease in accuracy for the local Gaussian state.



==> Evaluation_Over_Cutoff.tex <==

\begin{table*}
  \centering
    \begin{tabular}{lllrrrr}
    \toprule
     &  &  & \multicolumn{2}{r}{infidelity} & \multicolumn{2}{r}{evaluations} \\
     &  &  & mean & std & mean & std \\
    method & cutoff & layers &  &  &  &  \\
    \midrule
    \multirow[t]{12}{*}{CG} & \multirow[t]{3}{*}{3} & 1 & 0.391895 & 0.063252 & 161.200000 & 19.469634 \\
     &  & 2 & 0.275195 & 0.146968 & 261.900000 & 41.900544 \\
     &  & 3 & 0.312207 & 0.099059 & 402.400000 & 47.070160 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.442773 & 0.062790 & 155.300000 & 13.449907 \\
     &  & 2 & 0.310449 & 0.126411 & 289.100000 & 55.933393 \\
     &  & 3 & 0.407617 & 0.065311 & 392.600000 & 31.287910 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.452637 & 0.062186 & 153.400000 & 11.824645 \\
     &  & 2 & 0.395996 & 0.086296 & 278.900000 & 46.179481 \\
     &  & 3 & 0.363086 & 0.105192 & 385.000000 & 55.505755 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.455371 & 0.077067 & 144.400000 & 15.621922 \\
     &  & 2 & 0.403516 & 0.095972 & 271.100000 & 34.558967 \\
     &  & 3 & 0.443251 & 0.052907 & 386.777778 & 82.130655 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{COBYLA} & \multirow[t]{3}{*}{3} & 1 & 0.030078 & 0.025639 & 204.000000 & 7.133645 \\
     &  & 2 & 0.022656 & 0.034267 & 250.000000 & 0.000000 \\
     &  & 3 & 0.020020 & 0.032511 & 250.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.118066 & 0.195814 & 206.700000 & 6.377913 \\
     &  & 2 & 0.018750 & 0.026517 & 250.000000 & 0.000000 \\
     &  & 3 & 0.025293 & 0.029139 & 250.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.116113 & 0.194869 & 204.800000 & 7.161626 \\
     &  & 2 & 0.021777 & 0.027706 & 250.000000 & 0.000000 \\
     &  & 3 & 0.093457 & 0.150032 & 250.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.408496 & 0.205814 & 198.700000 & 5.735852 \\
     &  & 2 & 0.058789 & 0.139617 & 250.000000 & 0.000000 \\
     &  & 3 & 0.073134 & 0.101355 & 250.000000 & 0.000000 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{ImFil} & \multirow[t]{3}{*}{3} & 1 & 0.020215 & 0.015679 & 98.800000 & 3.155243 \\
     &  & 2 & 0.031250 & 0.028150 & 104.500000 & 5.482295 \\
     &  & 3 & 0.057324 & 0.039419 & 109.900000 & 6.226288 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.029395 & 0.023936 & 100.800000 & 3.583915 \\
     &  & 2 & 0.052051 & 0.028929 & 106.400000 & 5.460973 \\
     &  & 3 & 0.081348 & 0.062960 & 112.900000 & 9.255029 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.022559 & 0.021531 & 99.900000 & 3.478505 \\
     &  & 2 & 0.075684 & 0.039586 & 106.200000 & 4.848826 \\
     &  & 3 & 0.161816 & 0.050698 & 108.200000 & 6.828047 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.026270 & 0.016722 & 99.900000 & 3.381321 \\
     &  & 2 & 0.094629 & 0.073206 & 110.500000 & 4.972145 \\
     &  & 3 & 0.206814 & 0.101162 & 109.222222 & 8.303279 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{L-BFGS-B} & \multirow[t]{3}{*}{3} & 1 & 0.410449 & 0.061798 & 150.000000 & 34.985711 \\
     &  & 2 & 0.287402 & 0.153009 & 257.400000 & 36.739927 \\
     &  & 3 & 0.324609 & 0.104675 & 414.400000 & 67.651394 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.464746 & 0.062626 & 147.600000 & 19.431932 \\
     &  & 2 & 0.325781 & 0.135249 & 283.800000 & 31.026154 \\
     &  & 3 & 0.428613 & 0.068960 & 422.400000 & 67.546198 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.474707 & 0.061934 & 150.000000 & 35.888717 \\
     &  & 2 & 0.417090 & 0.092246 & 312.400000 & 76.068975 \\
     &  & 3 & 0.383496 & 0.105369 & 404.800000 & 60.363344 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.471680 & 0.079721 & 165.600000 & 52.092226 \\
     &  & 2 & 0.417480 & 0.094802 & 265.100000 & 48.768045 \\
     &  & 3 & 0.461697 & 0.058534 & 410.666667 & 71.105555 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{Nelder-Mead} & \multirow[t]{3}{*}{3} & 1 & 0.333008 & 0.125205 & 701.100000 & 21.717632 \\
     &  & 2 & 0.236523 & 0.153604 & 742.900000 & 55.921473 \\
     &  & 3 & 0.268262 & 0.108463 & 788.400000 & 44.754143 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.418164 & 0.060448 & 694.700000 & 14.514743 \\
     &  & 2 & 0.246680 & 0.151710 & 726.400000 & 43.665903 \\
     &  & 3 & 0.371484 & 0.066668 & 802.800000 & 34.653203 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.418457 & 0.060400 & 692.500000 & 25.382627 \\
     &  & 2 & 0.350586 & 0.096472 & 727.300000 & 41.231191 \\
     &  & 3 & 0.278223 & 0.173314 & 768.700000 & 71.019637 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.422559 & 0.082372 & 687.400000 & 15.931799 \\
     &  & 2 & 0.353906 & 0.128836 & 738.100000 & 40.311151 \\
     &  & 3 & 0.408203 & 0.056565 & 778.444444 & 45.047506 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{Powell} & \multirow[t]{3}{*}{3} & 1 & 0.004590 & 0.003713 & 617.100000 & 131.693626 \\
     &  & 2 & 0.006152 & 0.007366 & 1494.400000 & 563.312071 \\
     &  & 3 & 0.002832 & 0.002455 & 2090.600000 & 567.475345 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.003418 & 0.004046 & 676.400000 & 186.748910 \\
     &  & 2 & 0.008105 & 0.011078 & 1425.600000 & 431.032146 \\
     &  & 3 & 0.004883 & 0.004169 & 2482.600000 & 1040.292288 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.005078 & 0.005305 & 662.900000 & 183.404501 \\
     &  & 2 & 0.009375 & 0.012817 & 1322.500000 & 365.040104 \\
     &  & 3 & 0.002832 & 0.003270 & 2365.400000 & 610.574265 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.013965 & 0.021207 & 743.800000 & 298.516629 \\
     &  & 2 & 0.003320 & 0.003095 & 1454.500000 & 404.617858 \\
     &  & 3 & 0.014106 & 0.015725 & 2816.111111 & 836.283960 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{PyBobyqa} & \multirow[t]{3}{*}{3} & 1 & 0.076367 & 0.147462 & 100.000000 & 0.000000 \\
     &  & 2 & 0.019531 & 0.026139 & 100.000000 & 0.000000 \\
     &  & 3 & 0.201270 & 0.116866 & 100.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.183008 & 0.224018 & 100.000000 & 0.000000 \\
     &  & 2 & 0.023145 & 0.021411 & 100.000000 & 0.000000 \\
     &  & 3 & 0.303418 & 0.070709 & 100.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.303613 & 0.215337 & 100.000000 & 0.000000 \\
     &  & 2 & 0.102246 & 0.166126 & 100.000000 & 0.000000 \\
     &  & 3 & 0.260547 & 0.132003 & 100.000000 & 0.000000 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.377832 & 0.168647 & 100.000000 & 0.000000 \\
     &  & 2 & 0.144141 & 0.218906 & 100.000000 & 0.000000 \\
     &  & 3 & 0.371962 & 0.089228 & 100.000000 & 0.000000 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{12}{*}{SLSQP} & \multirow[t]{3}{*}{3} & 1 & 0.288672 & 0.157002 & 442.200000 & 142.646260 \\
     &  & 2 & 0.331836 & 0.111842 & 1128.600000 & 417.121672 \\
     &  & 3 & 0.377051 & 0.095819 & 1358.900000 & 967.647944 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{5} & 1 & 0.324219 & 0.178101 & 367.000000 & 174.943800 \\
     &  & 2 & 0.334863 & 0.138665 & 1068.700000 & 251.276762 \\
     &  & 3 & 0.354004 & 0.084963 & 1925.200000 & 663.078980 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{7} & 1 & 0.345898 & 0.146843 & 419.400000 & 122.675905 \\
     &  & 2 & 0.369141 & 0.133839 & 989.800000 & 427.039368 \\
     &  & 3 & 0.443359 & 0.052138 & 1713.900000 & 737.502610 \\
    \cline{2-7}
     & \multirow[t]{3}{*}{10} & 1 & 0.318555 & 0.178898 & 325.500000 & 196.658898 \\
     &  & 2 & 0.405566 & 0.067338 & 1012.000000 & 384.532328 \\
     &  & 3 & 0.429145 & 0.040905 & 1765.555556 & 777.821816 \\
    \cline{1-7} \cline{2-7}
    \bottomrule
\end{tabular}
\caption{Placeholder optimizer performance on  Local Gaussian state learning}
  \label{tab:1}
\end{table*}


\begin{table*}
  \centering
\begin{tabular}{lllrrrr}
    \toprule
     &  &  & \multicolumn{2}{r}{infidelity} & \multicolumn{2}{r}{evaluations} \\
     &  &  & mean & std & mean & std \\
     Cutoff & Layers & Optimizer &  &  &  &  \\
    \midrule
    \multirow[t]{4}{*}{3} & \multirow[t]{2}{*}{1} & COBYLA & 0.000084 & 0.000001 & 200.000000 & 0.000000 \\
     &  & Powell & 0.000084 & 0.000000 & 424.000000 & 128.693434 \\
    \cline{2-7}
     & \multirow[t]{2}{*}{2} & COBYLA & 0.046624 & 0.061800 & 200.000000 & 0.000000 \\
     &  & Powell & 0.000084 & 0.000000 & 2212.500000 & 1298.955157 \\
    \cline{1-7} \cline{2-7}
    \multirow[t]{4}{*}{4} & \multirow[t]{2}{*}{1} & COBYLA & 0.010940 & 0.008206 & 158.000000 & 59.396970 \\
     &  & Powell & 0.010900 & 0.008149 & 379.500000 & 256.679762 \\
    \cline{2-7}
     & \multirow[t]{2}{*}{2} & COBYLA & 0.008170 & 0.002585 & 200.000000 & 0.000000 \\
     &  & Powell & 0.001232 & 0.000170 & 2899.500000 & 499.924494 \\
    \cline{1-7} \cline{2-7}
    \bottomrule
\end{tabular}
\caption{Placeholder optimizer performance on  Non-Local Gaussian state learning}
  \label{tab:1}
\end{table*}
